An optimization-based approach to automated design

We propose a model-based, automated, bottom-up approach for design, which is applicable to various physical domains, but in this work we focus on the electrical domain. This bottom-up approach is based on a meta-topology in which each link is described by a universal component that can be instantiated as basic components (e.g., resistors, capacitors) or combinations of basic components via discrete switches. To address the combinatorial explosion often present in mixed-integer optimization problems, we present two algorithms. In the first algorithm, we convert the discrete switches into continuous switches that are physically realizable and formulate a parameter optimization problem that learns the component and switch parameters while inducing design sparsity through an $L_1$ regularization term. The second algorithm uses a genetic-like approach with selection and mutation steps guided by ranking of requirements costs, combined with continuous optimization for generating optimal parameters. We improve the time complexity of the optimization problem in both algorithms by reconstructing the model when components become redundant and by simplifying topologies through collapsing components and removing disconnected ones. To demonstrate the efficacy of these algorithms, we apply them to the design of various electrical circuits.

==> continuous_relaxation.tex <==
\section{Continuous relaxation with lossless realization}
When applying branch-and-bound heuristics to solve mixed integer programs, we end up in situations where the cost of the relaxation problem is better than the cost where the relaxed optimization variables are converted into integer variables. In this section we present a method where we avoid such a case. The key idea is the modeling interpretation of the switches that allow for their physical realization even in the case where they do not take integer values. In the universal component definition, each basic component as an associated switch that closes or opens a connection. When the switch is open, no current flows through the basic component, leading to the exclusion of that component from the design model. In the Modelica electrical library, the switch ({\tt Modelica.Electrical.Analog.Ideal.IdealOpeningSwitch}) is modeled such that when the switch is open, there is a large resistance that prevents the flow of the current. In contrast, when switch is close, there is a very small resistance that let the current flow unimpeded. This switch is controlled by a boolean input whose value determines the switch mode. We take inspiration from the definition of the Modelica switch and create a continuous switch that is controlled by a parameter that take values in [0, 1]. The switch is defined by the equations
\begin{eqnarray}
\label{eq:11021606}
  v &=& a((\varepsilon-1)s+1), \\
  \label{eq:11021608}
  i &=& a((1-\varepsilon)s+\varepsilon),
\end{eqnarray}
where $v$ is the switch voltage, $i$ is the current through the switch, $a$ is an auxiliary variable, $s\in [0,1]$ is the switch control, and $\varepsilon$ is a small hyper-parameter that determines the residual resistance when the switch is closed. The switch equation can be simplified to
$$v = \frac{(\varepsilon-1)s+1}{(1-\varepsilon)s+\varepsilon}i,$$
showing that for $s=0$ we have $v = i/{\varepsilon}$ and for $s=1$ we have $v = \varepsilon i$, the expected behavior of a switch. We do not use this simplified representation of the switch for numerical stability reasons. The introduction of the auxiliary variable $a$ avoids having equations with terms that can contain division by very small numbers. The drawback is that the resulting system of equations for the design model corresponds to a differential algebraic equation (DAE), rather than an ordinary differential equation (ODE). This consequence will affect the type of optimization approach we can use (see Section [ref] for more details). In addition to the requirements loss function $\mathcal{C}$  we introduce a sparsity $L_1$ regularization term, leading to the total optimization loss:
$$\mathcal{L}(\boldsymbol{p}, \boldsymbol{s}) = \mathcal{C}(\hat{\boldsymbol{y}}_{0:T}(\boldsymbol{p}, \boldsymbol{s}),\boldsymbol{y}_{0:T}) + \lambda \|\boldsymbol{s}\|_1,$$
where $0\leq {s}_i\leq 1$, with $\boldsymbol{s} = (s_i)$, and $\lambda$ is a positive weight that controls the sparsity strength. If in the optimization solution not all entries of $\boldsymbol{s}$ are zero or one, we map them into electric resistors with equivalent resistances, $\frac{(\varepsilon-1)s_i+1}{(1-\varepsilon)s_i+\varepsilon}$. Thus, we can physically realize them, without affecting the optimization cost function, i.e., the design requirements. We use a gradual approach to achieve sparsity. We start with a small $\lambda$ value to make sure that we generate an initial design that satisfies the requirements. Then we gradually increase $\lambda$ until the requirements cost function is no longer improved. Ideally, for each $\lambda$, we would like to obtain the optimal solution. However, it may take too many iterations to converge. Thus, for practical reasons, we limit the number of iterations for the optimization problem between alpha updates. The strategy for updating $\lambda$ is reminiscent to a primal-dual approach [ref], where we minimize $\mathcal{C}$ under an $L_1$ sparsity constraint. We could put a bound on the maximum number of components the design should have, i.e., $\|\boldsymbol{s}\|_1 - N_c\leq 0$, but it is unclear how to choose $N_c$ upfront. In our approach, we keep increasing $\lambda$ until we start harming the requirements cost function. When such an event occurs, we do not reduce the design model, even though some switch values have become zero, but continue with optimizing the current design. We eliminate box constraints via a variable transformation, to minimize $\mathcal{L}$ using a unconstrained optimization algorithm. For example, we eliminate a constrain of the form $a\leq x\leq b$, via the variable transformation $x = a + (\sin(\tilde{x}) + 1)(b-a)/2$, where $\tilde{x}$ is the new unconstrained optimization variable. The optimization solution is not guarantee to converge to a global minimizer, since we cannot asses any particular structure of the problem upfront due to the nonlinear dependence of the cost function on the optimization parameters. All optimization algorithm will require the evaluation of the design model. We use a black-box approach to optimization, where the cost evaluation is done by querying a computational model of the design: an FMU. In the cosimulation version of the FMU, such a representation contains in addition to the design description, the algorithm used for simulating the model (e.g., CVODE solver). FMUs can be integrated in several languages (e.g., Python, C, Java) and computational platforms (e.g., Matlab/Simulink, OpenModelica, Dymola).




==> solution_simplifications.tex <==
\section{Design solution simplifications}

==> stochastic_optimization.tex <==
\section{Stochastic optimization approach to control the combinatorial explosion}
 
